An Adversarial Active Sampling-based Data Augmentation Framework for Manufacturable Chip Design

Lithography modeling is a crucial problem in chip design to ensure a chip design mask is manufacturable. It requires rigorous simulations of optical and chemical models that are computationally expensive. Recent developments in machine learning have provided alternative solutions in replacing the time-consuming lithography simulations with deep neural networks. However, the considerable accuracy drop still impedes its industrial adoption. Most importantly, the quality and quantity of the training dataset directly affect the model performance. To tackle this problem, we propose a litho-aware data augmentation (LADA) framework to resolve the dilemma of limited data and improve the machine learning model performance. First, we pretrain the neural networks for lithography modeling and a gradient-friendly StyleGAN2 generator. We then perform adversarial active sampling to generate informative and synthetic in-distribution mask designs. These synthetic mask images will augment the original limited training dataset used to finetune the lithography model for improved performance. Experimental results demonstrate that LADA can successfully exploits the neural network capacity by narrowing down the performance gap between the training and testing data instances.

==> doc/prelim.tex <==
\section{Related Work}

\subsection{Machine Learning for Lithography Modeling}
Deep neural networks have been extensively studied for lithography modeling tasks. 
\cite{DFM-SPIE2019-Adam} is one of the very early attempts using machine learning for lithography modeling, 
where neural networks are designed to capture design critical dimensions.
\cite{DFM-DAC2019-Ye,DFM-ISPD2020-Ye} are representative GAN/U-Net-backboned solutions.
\cite{DFM-DAC2019-Ye,OPC-ICCAD2021-Chen} take the input of a mask image and generate the corresponding resist image, 
while \cite{DFM-ISPD2020-Ye} focuses on the optical modeling only.
Very recently, \cite{DFM-DAC2022-Yang} incorporates lithography physics into the neural network design and achieves the state-of-the-art performance on lithography modeling accuracy.

\subsection{Generative Adversarial Networks (GANs) in Data Augmentation}
Generative adversarial networks (GANs) composes of a generator and a discriminator neural network competing against each other to reach equilibrium during training, where the generator learns to generate realistic synthetic images trying to confuse the discriminators judgement from synthetic to real images. 
Following the seminar work of~\cite{GAN-NIPS2014-Goodefellow}, GANs attracted increasing attention both on improving the generated image quality and training stability~\cite{DCGAN-2015-Radford, WGAN-NIPS2017, ProgressiveGAN-2017, stylegan2}, as well as on a wide range of applications such as image-to-image translation~\cite{image-to-image}, super resolution~\cite{super-resolution}, and image inpainting~\cite{inpainting}.

Since GANs can generate realistic synthetic data with low cost, it has been quite popular as a data augmentation technique to avoid overfitting.
This has been especially helpful on application domains that do not have access to big data, such as medical imaging~\cite{medical-imaging}.
%In order for the generated data to be useful for downstream tasks, most works use conditioned GANs to produce labels along side with synthesized data.
In~\cite{liver-GAN}, the authors used Auxiliary Classifier Generative Adversarial Network~\cite{ACGAN} to synthesize CT images of liver lesions conditioned on each lesion category. 
Similarly for semantic segmentation tasks, CycleGAN~\cite{cylceGAN} is used to generate pixel-to-pixel mappings, either to form input and output image pairs used in the downstream segmentation network~\cite{cyleGAN-nature}.
%, cyleGAN-segmentation}.
Nonetheless, training downstream classifiers purely on synthetic images generated from GANs do still significantly underperform against classifiers trained on real images~\cite{gan-underperform, biggan-underperform}.

%Our work differs from prior work that leverages GANs in lithograph modeling in its fundamentals, where prior works~\cite{DFM-DAC2019-Ye,DFM-ISPD2020-Ye,OPC-ICCAD2021-Chen} mainly leverage GAN as the backbone to learn mappings between image domains, while our work uses GAN as a data augmentation technique to further boost the model accuracy.

\subsection{Adversarial Active Learning}
Active learning (AL) attempts to maximize model performance using the least amount of annotated samples as possible.
Active learning assumes that different data in the dataset holds different value for model improvement, and tries to select for the best data to improve the model performance.
AL approaches can be divided into membership query synthesis, stream-based selective sampling, and pool-based AL based on the application scenarios~\cite{active-learning-survey}.
Stream-based and pool-based differs only on how the unlabeled data is queried and labeled, either in data streams or on the entire unlabeled data pool.
Most work on AL adopts the pool-based scenario, since the unlabeled data pool can be easily obtained by artificially reserving a certain amount of data from popular machine learning datasets.
For membership query synthesis, the learner can request the label of any unlabeled dataset in the input domain, and this setting remains underexplored in the machine learning community.
Undoubtedly, membership query synthesis poses unique challenges in both producing realistic and diverse in distribution data, and often requires human-in-the-loop to obtain the ground truth labels~\cite{GAAL}.

We highlight that our work greatly differs from the previous line of work that use adversarial learning for active learning.
These works have leveraged adversarial representation learning as a sampling mechanism in active learning algorithms.
Specifically, the works of~\cite{VAAL, task-aware-VAAL} learns a latent space using a variational autoencoder and a adversarial network trained to distinguish between labeled and unlabeled data.
%The trained discriminator is used as a criterion, where samples in the unlabeled data pool that fool the discriminator are selected for active learning.

We coin our method as \textit{adversarial active sampling}, where adversarial comes from the term adversarial attack.
Adversarial attack aims at applying small perturbations to the original data, where the created adversarial examples would be misclassified by the original machine learning model~\cite{adversarial-attack}.
The work of~\cite{adversarial-sampling} use adversarial attack as a measure to approximate the distance to the classifier decision boundary, which is further used as a criterion to select active learning samples.
Our work closely resembles the work of~\cite{adversarial-active-sampling}, where we leverage adversarial attack as a ``benign'' method to create synthetic in-distribution unlabeled samples, which are most likely to corrupt the trained neural network results.
However, previous work~\cite{adversarial-active-sampling} only demonstrated adversarial sampling for pool-based settings for multi-class classification, where generated synthetic adversarial samples are used as guidance to select similar samples from the unlabeled pool.
In this work, our generated synthetic samples are used in a membership query-based active learning setting, and the downstream neural network is used for pixel-wise task, similar to semantic segmentation.

